Online Proximal-ADMM For Time-varying Constrained Convex Optimization

This paper considers a convex optimization problem with cost and constraints that evolve over time. The function to be minimized is strongly convex and possibly non-differentiable, and variables are coupled through linear constraints. In this setting, the paper proposes an online algorithm based on the alternating direction method of multipliers (ADMM), to track the optimal solution trajectory of the time-varying problem; in particular, the proposed algorithm consists of a primal proximal gradient descent step and an appropriately perturbed dual ascent step. The paper derives tracking results, asymptotic bounds, and linear convergence results. The proposed algorithm is then specialized to a multi-area power grid optimization problem, and our numerical results verify the desired properties.

==> Online Proximal-ADMM For Time-varyingConstrained Optimization/macro.tex <==
%\setlength{\textheight}{9.2in}
%\setlength{\textwidth}{6.75in}
%----------- for TF-07 -------------------
%\setlength{\textheight}{9.3in}
%\setlength{\textwidth}{6.8in}
%\addtolength{\topmargin}{-0.9in}
%\addtolength{\oddsidemargin}{-0.85in}
%-----------------------------------------
\setlength{\textheight}{9.1in}
\setlength{\textwidth}{6.6in}
\setlength{\topmargin}{0in}
\setlength{\oddsidemargin}{0in}
%for pdf
\addtolength{\topmargin}{-0.45in}
\addtolength{\oddsidemargin}{-0.06in}
%for ps
%\addtolength{\topmargin}{0.2in}
%\addtolength{\oddsidemargin}{-0.05in}
%
%
%-------- for times roman -----------------
%\renewcommand{\sfdefault}{phv}
%\renewcommand{\rmdefault}{ptm}
%\renewcommand{\ttdefault}{pcr}
%------------------------------------------
%----Platino-------------------------------
% \usepackage[sc]{mathpazo}
% \linespread{1.05}
% \selectfont
%------------------------------------------ 
%----helvet--------------------------------
%\usepackage{helvet}
%\renewcommand*\familydefault{\sfdefault}
%------------------------------------------
%------Arial-------------------------------
%\usepackage[T1]{fontenc}
%\usepackage[scaled]{uarial}
%\renewcommand*\familydefault{\sfdefault}
%------------------------------------------

%\parskip 1pt
%\leftmargini 1.5em 

%% The following commands reduce the size of section and
%% subsection headings from the original settings in article.cls
\makeatletter
\renewcommand\section{\@startsection {section}{1}{\z@}%
%                                  {-3.5ex \@plus -1ex \@minus -.2ex}%
                                   {-1.5ex \@plus -1ex \@minus -.1ex}%
%                                   {-2.0ex \@plus -1ex \@minus -.2ex}%
%                                   {2.3ex \@plus.2ex}%
%                                   {1.5ex \@plus.2ex}%
                                    {0.5ex \@plus.1ex}%
                                   {\normalfont\large\bfseries}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                     {-3.25ex\@plus -1ex \@minus -.2ex}%
%                                     {-2.0ex\@plus -1ex \@minus -.2ex}%
                                     {-1.0ex\@plus -1ex \@minus -.1ex}%
%                                     {1.5ex \@plus .2ex}%
%                                     {0.8ex \@plus .2ex}%
                                     {0.4ex \@plus .1ex}%
                                     {\normalfont\large\bfseries}}


%\newcommand{\nc}{\newcommand}
%\nc{\be}{\begin{equation}} \nc{\ee}{\end{equation}}
%\nc{\beqa}{\begin{eqnarray}} \nc{\eeqa}{\end{eqnarray}}
%\nc{\Av}{{\bf A}} \nc{\av}{{\bf a}} \nc{\Bv}{{\bf B}} \nc{\bv}{{\bf b}} 
%\nc{\Cv}{{\bf C}} \nc{\cv}{{\bf c}} \nc{\Dv}{{\bf D}} \nc{\dv}{{\bf d}} 
%\nc{\ev}{{\bf e}} \nc{\Ev}{{\bf E}} \nc{\Fv}{{\bf F}} \nc{\fv}{{\bf f}} 
%\nc{\gv}{{\bf g}} \nc{\Gv}{{\bf G}} \nc{\hv}{{\bf h}} \nc{\Hv}{{\bf H}} \nc{\Iv}{{\bf I}} 
%\nc{\Jv}{{\bf J}} \nc{\Lv}{{\bf L}} \nc{\lv}{{\mbox{\boldmath \em $l$}}} \nc{\Mv}{{\bf M}} \nc{\nv}{{\bf n}} 
%\nc{\zerov}{{\bf 0}} \nc{\Pv}{{\bf P}} \nc{\pv}{{\bf p}} 
%\nc{\Qv}{{\bf Q}} \nc{\qv}{{\bf q}} \nc{\Rv}{{\bf R}} 
%\nc{\rv}{{\bf r}} \nc{\Sv}{{\bf S}} \nc{\sv}{{\bf s}} 
%\nc{\Tv}{{\bf T}} \nc{\vv}{{\bf v}} \nc{\uv}{{\bf u}} 
%\nc{\Wv}{{\bf W}} \nc{\Uv}{{\bf U}} \nc{\Vv}{{\bf V}} 
%\nc{\wv}{{\bf w}} \nc{\Xv}{{\bf X}} \nc{\xv}{{\bf x}} 
%\nc{\yv}{{\bf y}} \nc{\zv}{{\bf z}}
%\nc{\sgn}{\mbox{sgn}}
%\def\barf{{{f}}} 
%\def\calC{{\mathcal{C}}}
%\def\calF{{\mathcal{F}}} 
%\def\calR{{\mathcal{R}}}
%\def\calS{{\mathcal{S}}}
%\def\calW{{\mathcal{W}}}	
%\def\calU{{\mathcal{U}}}
%\nc{\calPsi}{{\mathcal{\psi}}}
%\nc{\alphabf}{{\mbox{\boldmath $\alpha$}}}
%\nc{\betabf}{{\mbox{\boldmath $\beta$}}}
%\nc{\lambdabf}{{\mbox{\boldmath $\lambda$}}}
%\nc{\taubf}{{\mbox{\boldmath $\tau$}}}
%\nc{\mubf}{{\mbox{\boldmath $\mu$}}}
%\nc{\rhobf}{{\mbox{\boldmath $\rho$}}}
%\nc{\zetabf}{{\mbox{\boldmath $\zeta$}}}
%\nc{\phibf}{{\mbox{\boldmath $\phi$}}}
%\nc{\psibf}{{\mbox{\boldmath $\psi$}}}
%\nc{\diag}{\text{diag}}


==> macro.tex <==
%\setlength{\textheight}{9.2in}
%\setlength{\textwidth}{6.75in}
%----------- for TF-07 -------------------
%\setlength{\textheight}{9.3in}
%\setlength{\textwidth}{6.8in}
%\addtolength{\topmargin}{-0.9in}
%\addtolength{\oddsidemargin}{-0.85in}
%-----------------------------------------
\setlength{\textheight}{9.1in}
\setlength{\textwidth}{6.6in}
\setlength{\topmargin}{0in}
\setlength{\oddsidemargin}{0in}
%for pdf
\addtolength{\topmargin}{-0.45in}
\addtolength{\oddsidemargin}{-0.06in}
%for ps
%\addtolength{\topmargin}{0.2in}
%\addtolength{\oddsidemargin}{-0.05in}
%
%
%-------- for times roman -----------------
%\renewcommand{\sfdefault}{phv}
%\renewcommand{\rmdefault}{ptm}
%\renewcommand{\ttdefault}{pcr}
%------------------------------------------
%----Platino-------------------------------
% \usepackage[sc]{mathpazo}
% \linespread{1.05}
% \selectfont
%------------------------------------------ 
%----helvet--------------------------------
%\usepackage{helvet}
%\renewcommand*\familydefault{\sfdefault}
%------------------------------------------
%------Arial-------------------------------
%\usepackage[T1]{fontenc}
%\usepackage[scaled]{uarial}
%\renewcommand*\familydefault{\sfdefault}
%------------------------------------------

%\parskip 1pt
%\leftmargini 1.5em 

%% The following commands reduce the size of section and
%% subsection headings from the original settings in article.cls
\makeatletter
\renewcommand\section{\@startsection {section}{1}{\z@}%
%                                  {-3.5ex \@plus -1ex \@minus -.2ex}%
                                   {-1.5ex \@plus -1ex \@minus -.1ex}%
%                                   {-2.0ex \@plus -1ex \@minus -.2ex}%
%                                   {2.3ex \@plus.2ex}%
%                                   {1.5ex \@plus.2ex}%
                                    {0.5ex \@plus.1ex}%
                                   {\normalfont\large\bfseries}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                     {-3.25ex\@plus -1ex \@minus -.2ex}%
%                                     {-2.0ex\@plus -1ex \@minus -.2ex}%
                                     {-1.0ex\@plus -1ex \@minus -.1ex}%
%                                     {1.5ex \@plus .2ex}%
%                                     {0.8ex \@plus .2ex}%
                                     {0.4ex \@plus .1ex}%
                                     {\normalfont\large\bfseries}}


%\newcommand{\nc}{\newcommand}
%\nc{\be}{\begin{equation}} \nc{\ee}{\end{equation}}
%\nc{\beqa}{\begin{eqnarray}} \nc{\eeqa}{\end{eqnarray}}
%\nc{\Av}{{\bf A}} \nc{\av}{{\bf a}} \nc{\Bv}{{\bf B}} \nc{\bv}{{\bf b}} 
%\nc{\Cv}{{\bf C}} \nc{\cv}{{\bf c}} \nc{\Dv}{{\bf D}} \nc{\dv}{{\bf d}} 
%\nc{\ev}{{\bf e}} \nc{\Ev}{{\bf E}} \nc{\Fv}{{\bf F}} \nc{\fv}{{\bf f}} 
%\nc{\gv}{{\bf g}} \nc{\Gv}{{\bf G}} \nc{\hv}{{\bf h}} \nc{\Hv}{{\bf H}} \nc{\Iv}{{\bf I}} 
%\nc{\Jv}{{\bf J}} \nc{\Lv}{{\bf L}} \nc{\lv}{{\mbox{\boldmath \em $l$}}} \nc{\Mv}{{\bf M}} \nc{\nv}{{\bf n}} 
%\nc{\zerov}{{\bf 0}} \nc{\Pv}{{\bf P}} \nc{\pv}{{\bf p}} 
%\nc{\Qv}{{\bf Q}} \nc{\qv}{{\bf q}} \nc{\Rv}{{\bf R}} 
%\nc{\rv}{{\bf r}} \nc{\Sv}{{\bf S}} \nc{\sv}{{\bf s}} 
%\nc{\Tv}{{\bf T}} \nc{\vv}{{\bf v}} \nc{\uv}{{\bf u}} 
%\nc{\Wv}{{\bf W}} \nc{\Uv}{{\bf U}} \nc{\Vv}{{\bf V}} 
%\nc{\wv}{{\bf w}} \nc{\Xv}{{\bf X}} \nc{\xv}{{\bf x}} 
%\nc{\yv}{{\bf y}} \nc{\zv}{{\bf z}}
%\nc{\sgn}{\mbox{sgn}}
%\def\barf{{{f}}} 
%\def\calC{{\mathcal{C}}}
%\def\calF{{\mathcal{F}}} 
%\def\calR{{\mathcal{R}}}
%\def\calS{{\mathcal{S}}}
%\def\calW{{\mathcal{W}}}	
%\def\calU{{\mathcal{U}}}
%\nc{\calPsi}{{\mathcal{\psi}}}
%\nc{\alphabf}{{\mbox{\boldmath $\alpha$}}}
%\nc{\betabf}{{\mbox{\boldmath $\beta$}}}
%\nc{\lambdabf}{{\mbox{\boldmath $\lambda$}}}
%\nc{\taubf}{{\mbox{\boldmath $\tau$}}}
%\nc{\mubf}{{\mbox{\boldmath $\mu$}}}
%\nc{\rhobf}{{\mbox{\boldmath $\rho$}}}
%\nc{\zetabf}{{\mbox{\boldmath $\zeta$}}}
%\nc{\phibf}{{\mbox{\boldmath $\phi$}}}
%\nc{\psibf}{{\mbox{\boldmath $\psi$}}}
%\nc{\diag}{\text{diag}}

